Trajectory-User Linking via Hierarchical Spatio-Temporal Attention Networks

Trajectory-User Linking (TUL) is crucial for human mobility modeling by linking diferent trajectories to users with the exploration of complex mobility patterns. Existing works mainly rely on the recurrent neural framework to encode the temporal dependencies in trajectories, have fall short in capturing spatial-temporal global context for TUL prediction. To ill this gap, this work presents a new hierarchical spatio-temporal attention neural network, called AttnTUL, to jointly encode the local trajectory transitional patterns and global spatial dependencies for TUL. Speciically, our irst model component is built over the graph neural architecture to preserve the local and global context and enhance the representation paradigm of geographical regions and user trajectories. Additionally, a hierarchically structured attention network is designed to simultaneously encode the intra-trajectory and inter-trajectory dependencies, with the integration of the temporal attention mechanism and global elastic attentional encoder. Extensive experiments demonstrate the superiority of our AttnTUL method as compared to state-of-the-art baselines on various trajectory datasets. The source code of our model is available at https://github.com/Onedean/AttnTUL.

==> table/algorithm_grid.tex <==
\begin{algorithm}
    \caption{Trajectories to Grids}
    \fontsize{10}{14}\selectfont
    \renewcommand{\algorithmicrequire}{ \textbf{Input:}}
    \renewcommand{\algorithmicensure}{ \textbf{Output:}}
    \begin{algorithmic}[1]
        \REQUIRE ~~\\
            The set of trajectory: $\textbf{T}$\\
            The set area: $Lon_{min},Lon_{max},Lat_{min},Lon_{max}$\\
            The size of grid: $d$
        \ENSURE ~~\\
            Grid sequence corresponding to trajectory $\textbf{T}$: $\textbf{L}$
        
        \STATE $//$ Compute the distance of area by Haversine formula
        \STATE $length = Haversine(Lon_{min},Lat_{min},Lon_{max},Lat_{min})$
        \STATE $width = Haversine(Lon_{min},Lat_{min},Lon_{min},Lat_{max})$
        \STATE $//$ Compute the number of grids in longitude/latitude
        \STATE $N_{lon} = \frac{length}{d}$
        \STATE $N_{lat} = \frac{width}{d}$
        \STATE $//$ Compute the gap of a grid in longitude/latitude
        \STATE $g_{lon} = \frac{Lon_{max}-Lon_{min}}{N_{lon}}$
        \STATE $g_{lat} = \frac{Lat_{max}-Lat_{min}}{N_{lat}}$
        
        \FOR{$<lon,lat>$ in $\textbf{T}$}
            \STATE $id=\frac{(lat-Lat_{min})*N_{lon}}{g_{lat}}+\frac{lon-Lon_{min}}{g_{lon}}$
            \STATE add $id$ to list $V$
        \ENDFOR
        \STATE List $V$ drops duplicates and sorts to get a new list $V_{new}$
        \FOR{$v$ in $V$}
            \STATE find the index $idx$ of $v$ in the list $V_{new}$
            \STATE add $idx$ to list $\textbf{L}$
        \ENDFOR
        \RETURN $\textbf{L}$
    \end{algorithmic}
\end{algorithm}

==> table/method_compared.tex <==
\begin{table}
    \caption{Advantages compared with existing methods}
    \label{tab:compared}
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \centering
    \fontsize{6}{12}\selectfont
    \begin{tabular}{l|l|l|l}
    & Dataset type & Track length & Mining mode\\
    \hline
    Classical & \tabincell{l}{LBSNs} & \tabincell{l}{Short} & \tabincell{c}{Sequential / Spatial}\\
    RNN-based & \tabincell{l}{LBSNs} & \tabincell{l}{Short / Medium} & \tabincell{l}{Sequential / Spatial / Temporal}\\
    \hline
    This work & \tabincell{l}{LBSNs / LBS} & \tabincell{l}{Short / Medium / Long} & \tabincell{l}{Sequential / State
    \\Multi-scale Spatial / Temporal}\\
    \end{tabular}\vspace{0cm}
\end{table}

==> table/param_set.tex <==
\begin{table}
    \caption{Typical parameter settings.}
    \label{tab:param_set}
    \centering
    \fontsize{8}{12}\selectfont
    \begin{tabular}{cccccc}
    \toprule[1pt]
    Item & Choose & Range & Feature & Choose & Range\\
    \cmidrule(r){1-3}\cmidrule(r){4-6}
    batch size & 16 & 1-64 & grid & 128 & 32-512\\
    learning rate & 0.001 & 0.0005-0.005 & time & 32 & 16-128\\
    drop out & 0.5 & 0-1 & state & 32 & 16-128\\
    Stacked & 3 & 2-4 & location & 128 & 16-512\\
    \bottomrule[1pt]
    \end{tabular}
\end{table}

==> table/time.tex <==
\begin{table}[t]
% \vspace{-7mm}
\centering
\caption{Efficiency Evaluation}
\label{tab:time}
% \vspace{-2mm}
\fontsize{9}{12} \selectfont
\hspace{-6mm}
\setlength{\tabcolsep}{1.35mm}{}
\begin{tabular}{c|c|c|c}
\toprule

Data & Methods & Training Time/per epoch & Inference Time\\

\midrule

\multirow{12}{*}{\rotatebox{90}{Gowalla ($|\mathcal{U}|$=222)}} & LCSS & -  & 565\\ \cline{2-4}

& LDA & - & 578\\
\cline{2-4}

& DT & - & 634\\ 
\cline{2-4}

& SR & - & 268\\
\cline{2-4}

& TULER-L & 1.33 & 0.28\\
\cline{2-4}

& TULER-G & 1.23 & 0.25\\
\cline{2-4}

& Bi-TULER & 1.88 & 0.33\\
\cline{2-4}

& TULVAE & 13.52 & 1.85\\
\cline{2-4}

& DeepTUL & - & -\\
\cline{2-4}

& DPLink & 1.83 & 0.34\\
\cline{2-4}
& T3S & 10.23 & 0.92\\
\cline{2-4}
& \model & 5.26 & 1.71 \\

\bottomrule

\end{tabular}
% \vspace{-1mm}
\end{table}
